Rate Splitting for Massive MIMO Multi-carrier system using Full Duplex Decode and Forward Relay with Hardware Impairments

In this paper, we address the power allocation problem for a decode and forward (DF) relay system, where a massive multiple-input-multiple-output (mMIMO) multi-carrier (MC) base station (BS) node communicates with a MC single antenna node directly and also through the single antenna full duplex (FD) MC relay, using rate splitting (RS) approach. Successive interference cancellation approach is adopted at the destination. We consider orthogonal frequency division multiplexing (OFDM) as our MC strategy. We take into account the impact of hardware distortions resulting in residual self-interference and inter-carrier leakage (ICL), and also imperfect channel state information (CSI). We formulate a joint sub-carrier and power allocation problem to maximize the total sum rate. An iterative optimization method is proposed, which follows successive inner approximation (SIA) framework to reach the convergence point that satisfies the Karush-Kuhn-Tucker (KKT) conditions. Numerical results show the significance of distortion-aware design for such systems, and also the significant gain in terms of sum rate compared to its half duplex (HD) and also non-rate splitting scheme.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{xstring}
\usepackage{dsfont}
\usepackage{amssymb}
% \usepackage{amsthm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% MAIN MACROS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\def\alphabet{abcdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRST123456789}
\renewcommand{\vec}[1]{
	\IfSubStr{\alphabet}{#1}{
		\ensuremath{\mbf{\MakeLowercase{#1}}}
	}{
		\ensuremath{\bm{\MakeLowercase{#1}}}
	}
}
\newcommand{\mat}[1]{
	\IfSubStr{\alphabet}{#1}{
		\ensuremath{\mathbf{\MakeUppercase{#1}}}
	}{
		\ensuremath{\boldsymbol{\MakeUppercase{#1}}}
	}
}
\newcommand{\set}[1]{\ensuremath{\mathcal{\MakeUppercase{#1}}}}
\newcommand{\dist}[1]{\ensuremath{P_{\MakeUppercase{#1}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% THEOREMS, LEMMAS, ETC %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{remark}{Remark}
% \newtheorem{proof}{Proof}
% \newtheorem{definition}{Definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% WELL-KNOWN SYMBOLS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\T{\mathsf{T}}
\def\R{\mathbb R}
\def\Z{\mathbb Z}
\def\E{\mathbb E}
\def\P{\mathbb P}
\def\N{\mathbb N}
\def\F{\mathsf{F}}
\def\KL{D_\mathrm{KL}}
\def\ord{\mcl O}
\def\vectorize{\mathrm{vec}}
\def\Bern{\mathrm{Bern}}
\def\Var{\mathrm{Var}}
\def\Cov{\mathrm{Cov}}
\renewcommand\epsilon{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% OPERATORS (),[],{}, ... %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ceq}[1]{\overset{#1}{=}}
\newcommand{\cgeq}[1]{\overset{#1}{\geq}}
\newcommand{\cleq}[1]{\overset{#1}{\leq}}
\newcommand{\cl}[1]{\overset{#1}{<}}
\newcommand{\cg}[1]{\overset{#1}{>}}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\mcl}{\mathcal}
\newcommand{\mrm}{\mathrm}
\newcommand{\bld}{\boldsymbol}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand*{\inner}[2]{\left\langle#1,#2\right\rangle}
\newcommand*{\norm}[1]{\left\|#1\right\|}
\newcommand*{\parents}[1]{\left(#1\right)}
\newcommand*{\braces}[1]{\left\{#1\right\}}
\newcommand*{\brackets}[1]{\left[#1\right]}
\newcommand*{\card}[1]{\left|#1\right|}
\newcommand*{\abs}[1]{\left|#1\right|}
\newcommand*{\floor}[1]{\left\lfloor #1 \right\rfloor}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmax}{argmax}
\let\ab\allowbreak

%% To avoid conflicts with ICLR templates
\newcommand{\citet}[1]{\cite{#1}}
\newcommand{\citep}[1]{\cite{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% MACROS WITH MEANING %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\defeq{:=}
\def\d{\mathrm{d}} 
\def\margin{\ensuremath{\nu}}
\def\datadist{\mathcal D}
\def\nclasses{\ensuremath{k}}
\def\inputdim{\ensuremath{n}}
\def\ntrainsamples{\ensuremath{m}}
\def\trainloss{\set{L}}
\def\ball{\set{B}}
\newcommand*{\ind}[1]{\mathds{1}\left(#1\right)}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% SHORTCUTS (OPTIONAL) %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Vectors
\def\vzero{\vec{0}}
\def\1{\vec{1}}
\def\vone{\vec{1}}
\def\vmu{\vec{\mu}}
\def\vtheta{\vec{\theta}}
\def\veta{\vec{\eta}}
\def\vpi{\vec{\pi}}
\def\va{\vec{a}}
\def\vb{\vec{b}}
\def\vc{\vec{c}}
\def\vd{\vec{d}}
\def\ve{\vec{e}}
\def\vf{\vec{f}}
\def\vg{\vec{g}}
\def\vh{\vec{h}}
\def\vi{\vec{i}}
\def\vj{\vec{j}}
\def\vk{\vec{k}}
\def\vl{\vec{l}}
\def\vm{\vec{m}}
\def\vn{\vec{n}}
\def\vo{\vec{o}}
\def\vp{\vec{p}}
\def\vq{\vec{q}}
\def\vr{\vec{r}}
\def\vs{\vec{s}}
\def\vt{\vec{t}}
\def\vu{\vec{u}}
\def\vv{\vec{v}}
\def\vw{\vec{w}}
\def\vx{\vec{x}}
\def\vy{\vec{y}}
\def\vz{\vec{z}}

% Matrix
\def\mone{\mat{1}}
\def\mzero{\mat{0}}
\def\mA{\mat{A}}
\def\mB{\mat{B}}
\def\mC{\mat{C}}
\def\mD{\mat{D}}
\def\mE{\mat{E}}
\def\mF{\mat{F}}
\def\mG{\mat{G}}
\def\mH{\mat{H}}
\def\mI{\mat{I}}
\def\mJ{\mat{J}}
\def\mK{\mat{K}}
\def\mL{\mat{L}}
\def\mM{\mat{M}}
\def\mN{\mat{N}}
\def\mO{\mat{O}}
\def\mP{\mat{P}}
\def\mQ{\mat{Q}}
\def\mR{\mat{R}}
\def\mS{\mat{S}}
\def\mT{\mat{T}}
\def\mU{\mat{U}}
\def\mV{\mat{V}}
\def\mW{\mat{W}}
\def\mX{\mat{X}}
\def\mY{\mat{Y}}
\def\mZ{\mat{Z}}
\def\mBeta{\mat{\beta}}
\def\mPhi{\mat{\Phi}}
\def\mLambda{\mat{\Lambda}}
\def\mSigma{\mat{\Sigma}}
\def\mPi{\mat{\Pi}}

% Sets
\def\sA{\set{A}}
\def\sB{\set{B}}
\def\sC{\set{C}}
\def\sD{\set{D}}
\def\sE{\set{E}}
\def\sF{\set{F}}
\def\sG{\set{G}}
\def\sH{\set{H}}
\def\sI{\set{I}}
\def\sJ{\set{J}}
\def\sK{\set{K}}
\def\sL{\set{L}}
\def\sM{\set{M}}
\def\sN{\set{N}}
\def\sO{\Theta}
\def\sP{\set{P}}
\def\sQ{\set{Q}}
\def\sR{\set{R}}
\def\sS{\set{S}}
\def\sT{\set{T}}
\def\sU{\set{U}}
\def\sV{\set{V}}
\def\sW{\set{W}}
\def\sX{\set{X}}
\def\sY{\set{Y}}
\def\sZ{\set{Z}}

% Distribution of []
% Sets
\def\distA{\dist{A}}
\def\distB{\dist{B}}
\def\distC{\dist{C}}
\def\distD{\dist{D}}
\def\distE{\dist{E}}
\def\distF{\dist{F}}
\def\distG{\dist{G}}
\def\distH{\dist{H}}
\def\distI{\dist{I}}
\def\distJ{\dist{J}}
\def\distK{\dist{K}}
\def\distL{\dist{L}}
\def\distM{\dist{M}}
\def\distN{\dist{N}}
\def\distO{\dist{O}}
\def\distP{\dist{P}}
\def\distQ{\dist{Q}}
\def\distR{\dist{R}}
\def\distS{\dist{S}}
\def\distT{\dist{T}}
\def\distU{\dist{U}}
\def\distV{\dist{V}}
\def\distW{\dist{W}}
\def\distX{\dist{X}}
\def\distY{\dist{Y}}
\def\distZ{\dist{Z}}


%% Nodes and Channels
\def\sr{\text{sr}}
